Generative Mask Pyramid Network for CT/CBCT Metal Artifact Reduction with Joint Projection-Sinogram Correction

A conventional approach to computed tomography (CT) or cone beam CT (CBCT) metal artifact reduction is to replace the X-ray projection data within the metal trace with synthesized data. However, existing projection or sinogram completion methods cannot always produce anatomically consistent information to fill the metal trace, and thus, when the metallic implant is large, significant secondary artifacts are often introduced. In this work, we propose to replace metal artifact affected regions with anatomically consistent content through joint projection-sinogram correction as well as adversarial learning. To handle the metallic implants of diverse shapes and large sizes, we also propose a novel mask pyramid network that enforces the mask information across the network's encoding layers and a mask fusion loss that reduces early saturation of adversarial training. Our experimental results show that the proposed projection-sinogram correction designs are effective and our method recovers information from the metal traces better than the state-of-the-art methods.

==> figures/checkerboard_effect.tex <==
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{.49\linewidth}
%       \includegraphics[width=\textwidth]{figures/data/checkerboard_effect_col_0.png}
%       \caption{Sinogram}
%     \end{subfigure}
%     \begin{subfigure}[b]{.49\linewidth}
%         \includegraphics[width=\textwidth]{figures/data/checkerboard_effect_col_1.png}
%         \caption{CT}
%     \end{subfigure}
%     \caption{Sinogram completion and CT reconstruction results with and without checkerboard artifact correction. Rows: (1) without MAR, (2) ground truth, (3) without checkerboard artifact correction, and (4) with checkerboard artifact correction. The yellow contours outline the regions affected by metal implants.}
%     \label{fig:checkerboard_effect}
% \end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{.24\linewidth}
      \includegraphics[width=\textwidth]{figures/data/checkerboard_sino_input.png}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
      \includegraphics[width=\textwidth]{figures/data/checkerboard_sino_gt.png}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
      \includegraphics[width=\textwidth]{figures/data/checkerboard_sino_with.png}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
      \includegraphics[width=\textwidth]{figures/data/checkerboard_sino_without.png}
    \end{subfigure}
    \vspace{0.2em}
    \begin{subfigure}[b]{.24\linewidth}
      \includegraphics[width=\textwidth]{figures/data/checkerboard_ct_input.png}
      \caption{}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
      \includegraphics[width=\textwidth]{figures/data/checkerboard_ct_gt.png}
      \caption{}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
      \includegraphics[width=\textwidth]{figures/data/checkerboard_ct_with.png}
      \caption{}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
      \includegraphics[width=\textwidth]{figures/data/checkerboard_ct_without.png}
      \caption{}
    \end{subfigure}

    \caption{Sinogram completion (top) and CT reconstruction (bottom) results with and without checkerboard artifact correction. (a) without MAR, (b) ground truth, (c) w/o checkerboard artifact correction, and (d) w/ checkerboard artifact correction. The yellow contours outline the regions affected by metal implants.}
    \label{fig:checkerboard_effect}
\end{figure}
  

==> figures/compare_mask_focused.tex <==
\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{.19\linewidth}
    \includegraphics[width=\textwidth]{figures/data/blob_masked_col_0.png}
    \caption{Masked}
\end{subfigure}
\begin{subfigure}[b]{.19\linewidth}
    \includegraphics[width=\textwidth]{figures/data/blob_masked_col_1.png}
    \caption{Unmasked}
\end{subfigure}
  \begin{subfigure}[b]{.19\linewidth}
      \includegraphics[width=\textwidth]{figures/data/blob_masked_col_2.png}
      \caption{LI}
  \end{subfigure}
  \begin{subfigure}[b]{.19\linewidth}
      \includegraphics[width=\textwidth]{figures/data/blob_masked_col_3.png}
      \caption{BF}
  \end{subfigure}
  \begin{subfigure}[b]{.19\linewidth}
    \includegraphics[width=\textwidth]{figures/data/blob_masked_col_4.png}
    \caption{MFL}
\end{subfigure}
  \caption{Visual comparison of models completing blob-masked X-ray projections. A colormap is applied for improved details of the bone region.}
  \label{fig:compare_mask_focused}
\end{figure*}

==> figures/compare_mask_recalled.tex <==
\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{.19\linewidth}
    \includegraphics[width=\textwidth]{figures/data/metal_masked_col_0.png}
    \caption{Masked}
\end{subfigure}
\begin{subfigure}[b]{.19\linewidth}
    \includegraphics[width=\textwidth]{figures/data/metal_masked_col_1.png}
    \caption{Unmasked}
\end{subfigure}
  \begin{subfigure}[b]{.19\linewidth}
      \includegraphics[width=\textwidth]{figures/data/metal_masked_col_2.png}
      \caption{MFL-blob}
  \end{subfigure}
  \begin{subfigure}[b]{.19\linewidth}
      \includegraphics[width=\textwidth]{figures/data/metal_masked_col_3.png}
      \caption{MFL-metal}
  \end{subfigure}
  \begin{subfigure}[b]{.19\linewidth}
    \includegraphics[width=\textwidth]{figures/data/metal_masked_col_4.png}
    \caption{PC}
\end{subfigure}
  \caption{Visual comparison of models completing metal-masked X-ray projections. A colormap is applied for improved details of the bone region.}
  \label{fig:compare_mask_recalled}
\end{figure*}

==> figures/simulated_images.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{.16\linewidth}
      \includegraphics[width=\textwidth]{figures/data/clean.png}
    %   \caption{Without artifact}
  \end{subfigure}
  \begin{subfigure}[b]{.16\linewidth}
      \includegraphics[width=\textwidth]{figures/data/metal_low.png}
    %   \caption{Mild artifact}
  \end{subfigure}
    \begin{subfigure}[b]{.16\linewidth}
        \includegraphics[width=\textwidth]{figures/data/metal_high.png}
        % \caption{Severe artifact}
    \end{subfigure}
    \caption{Sample CBCT images with (a) no, (b) mild, and (c) severe artifact.}
    \label{fig:simulated_images}
\end{figure}
  

==> figures/sinogram_refine.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{.24\linewidth}
        \includegraphics[width=\textwidth]{figures/data/sinogram_refine_col_0.png}
        \caption{Masked}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
        \includegraphics[width=\textwidth]{figures/data/sinogram_refine_col_1.png}
        \caption{Unmasked}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
        \includegraphics[width=\textwidth]{figures/data/sinogram_refine_col_2.png}
        \caption{PC}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
        \includegraphics[width=\textwidth]{figures/data/sinogram_refine_col_3.png}
        \caption{PC+SC}
    \end{subfigure}
    \caption{Projection (top) and sinogram (bottom) completion results with and without SC. A colormap is applied for improved details of the bone region.}
    \label{fig:sinogram_refine}
  \end{figure}

==> figures/ssim_rmse.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{l | c c c c c c c}
\hline
   &   Original   &   LI          & BHC        & NMAR1       &  NMAR2     &  CNNMAR    & Ours \\
\hline
Mild Artifact &   00.0/00.0  &   00.0/00.0   & 00.0/00.0  & 00.0/00.0   &  00.0/00.0 &  00.0/00.0 & 00.0/00.0  \\
Severe Artifact &   00.0/00.0  &   00.0/00.0   & 00.0/00.0  & 00.0/00.0   &  00.0/00.0 &  00.0/00.0 & 00.0/00.0  \\
\hline
Average &   00.0/00.0  &   00.0/00.0   & 00.0/00.0  & 00.0/00.0   &  00.0/00.0 &  00.0/00.0 & 00.0/00.0  \\
\hline
\end{tabular}
\caption{SSIM and RMSE (HU) performance comparisons (SSIM/RMSE).}
\label{table:comparison}
\end{table*}
